ABot-Earth 0.5: Generative 3D Earth Model

We present ABot-Earth 0.5, a generative 3D framework designed to synthesize vast, seamless 3D environments from ubiquitous, geospatially referenced satellite imagery. To achieve this, we propose a novel generative model formulated directly with the 3D Gaussian Splatting (3DGS) representation. The model is trained on a diverse corpus of existing real-world urban reconstructions, learning to generate realistic geometry and textures. At inference, it synthesizes novel 3D scenes conditioned solely on satellite imagery at a scalable rate of under 10 minutes per square kilometer, while demonstrating exceptional realism. The framework is designed for accessibility, with integrated hierarchical level-of-detail (LOD) structures that permit real-time, interactive visualization on web-based map engines. This high-fidelity simulation sandbox effectively mitigates the sim-to-real domain gap, enabling critical downstream Embodied AI applications like closed-loop UAV navigation. By providing an ultra-low-cost and high-efficiency solution, ABot-Earth 0.5 significantly lowers the technical and financial barriers to large-scale 3D reconstruction and empowers the future of global digital earth visualization.

==> body/table_tex/intro_compare.tex <==

\begin{table*}[t]
\centering
\caption{Comparison of 3D Earth/city generation methods. Our method is trained directly on real-world 3DGS data with single-image conditioning, enabling large-scale generation without seam artifacts. Inference speed is reported as a coarse qualitative estimate of the time required to synthesize approximately 1\,km$^2$ of scene content.}
\label{tab:comparison}
\vspace{-0.5em}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccc}
\begin{tabular}{l l l l l l p{1.2cm}}
\toprule
\textbf{Method} & \textbf{Training Data} & \textbf{Condition} & \textbf{Beyond Buildings} & \textbf{Large-Scale} & \textbf{Core Paradigm} & \textbf{Speed} \\
\midrule
Sat2Scene~\cite{sat2scene} & Images \& Height Map & Layout & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & Geo. Coloring & / \\
Sat2City~\cite{sat2city} & Mesh & Height Map & \textcolor{red}{\ding{55}} & {\color{green}\checkmark} & Building Object Gen. & / \\
Sat2Density++~\cite{Qian_2026_Sat2Densitypp} & Images & Single Satellite & {\color{green}\checkmark} & \textcolor{red}{\ding{55}} & Feedforward & / \\
Sat3DGen~\cite{qian2026satdgen} & Images & Single Satellite & {\color{green}\checkmark} & \textcolor{red}{\ding{55}} & Feedforward & / \\
UrbanWorld~\cite{urbanworld} & Mesh + UV & OSM or Layout & {\color{green}\checkmark} & {\color{green}\checkmark} & Multi-Stage & / \\
SynCity~\cite{engstler2025syncity} & Training Free & Text Prompt & {\color{green}\checkmark} & {\color{green}\checkmark} & Multi-Stage & / \\
SkyFall-GS~\cite{skyfallgs} & Images & Multi-view Satellite & {\color{green}\checkmark} & {\color{green}\checkmark} & Iterative Optimization & 6 hours \\
Orbit2Ground~\cite{orbit2ground} & Images & Multi-view Satellite & {\color{green}\checkmark} & {\color{green}\checkmark} & Iterative Optimization & / \\
XCube~\cite{ren2024xcube} & Mesh & LiDAR Scan & {\color{green}\checkmark} & {\color{green}\checkmark} & 3D Generative & N/A \\
EarthCrafter~\cite{earthcrafter} & Mesh & Satellite + Depth & {\color{green}\checkmark} & {\color{green}\checkmark} & 3D Generative & 2 hours \\
\midrule
\textbf{Ours} & \textbf{3DGS} & \textbf{Single Satellite} & \textbf{\textcolor{green}{\checkmark}} & \textbf{\textcolor{green}{\checkmark}} & \textbf{3D Generative} & \textbf{10 min} \\
\bottomrule
\end{tabular}%
}
% \vspace{0.5em}
\end{table*}


==> body/table_tex/large_scale_efficiency.tex <==
\begin{table}[h]
\centering
\caption{Efficency comparison of different products.}
\vspace{-0.5em}
\label{tab:large_scale_efficiency}
\begin{tabular}{l c c c}
\toprule
Method & Cost $\downarrow$ & Freshness $\downarrow$ & Storage $\downarrow$ \\
\midrule
Marble & -- & -- & -- \\
Google-Earth & High & Month & GB \\
\textbf{ABot-Earth(Ours)} & \textbf{Free} & \textbf{Day} & \textbf{MB} \\
\bottomrule
\end{tabular}
\end{table}

==> body/table_tex/opendataset.tex <==
\begin{table}[t]
\centering
\caption{Open-source city-scale datasets incorporated in our training pipeline.
\checkmark\ indicates the attribute is available.}
\label{tab:open_datasets}
\small
\begin{tabular}{l r r c c c c c c c}
\toprule
\textbf{Dataset} & \textbf{Images} & \textbf{Area} & \textbf{DOF} & \textbf{Viewpoint} & \textbf{Aerial Type} & \textbf{Depth} & \textbf{Weather} & \textbf{Light} & \textbf{Seq.} \\
\midrule
\multicolumn{10}{l}{\textit{Synthetic City-Scale}} \\
\addlinespace[2pt]
AerialGo        & 3.45M & 134\,km$^2$   & 6 & UAV+Ground   & Oblique   & \checkmark & \checkmark & \checkmark & \checkmark \\
MatrixCity      & 519K  & 28\,km$^2$    & 6 & UAV+Ground   & Arbitrary & \checkmark & \checkmark & \checkmark & \checkmark \\
MatrixCity-Sat  & 50    & 1\,km$^2$     & / & Satellite    & Near-nadir & \checkmark & --         & --         & -- \\
\addlinespace[4pt]
\multicolumn{10}{l}{\textit{Real-World City-Scale}} \\
\addlinespace[2pt]
UrbanScene3D    & 128K  & 55\,km$^2$    & 6 & UAV          & Arbitrary & \checkmark & --         & --         & \checkmark \\
UrbanBIS        & 113K  & 10.78\,km$^2$ & 3 & UAV          & Arbitrary & --         & --         & --         & \checkmark \\
CrossLoc        & 57K   & 2.7\,km$^2$   & 6 & UAV          & Arbitrary & \checkmark & --         & --         & \checkmark \\
Mill-19         & 3.5K  & 0.18\,km$^2$  & 6 & UAV          & Overhead  & --         & --         & \checkmark & \checkmark \\
UAVD4L          & 0.3K  & 2.5\,km$^2$   & 6 & UAV          & Arbitrary & \checkmark & --         & --         & \checkmark \\
Demo UAV        & 27K   & --            & / & Sat.+UAV     & --        & --         & --         & --         & -- \\
\addlinespace[4pt]
\multicolumn{10}{l}{\textit{Real-World Satellite}} \\
\addlinespace[2pt]
DFC 2019        & --    & $\sim$4\,km$^2$ & / & Satellite (WV-3) & Off-nadir & --     & --         & --         & -- \\
GoogleEarth     & --    & $\sim$4\,km$^2$ & / & Satellite+Ground & Mixed    & --     & --         & \checkmark & -- \\
\addlinespace[4pt]
\multicolumn{10}{l}{\textit{Satellite / Cross-View}} \\
\addlinespace[2pt]
CVUSA           & 88K   & --            & / & Sat.+Ground  & --        & --         & --         & --         & -- \\
CVACT           & 256K  & --            & / & Sat.+Ground  & --        & --         & --         & --         & -- \\
VIGOR           & 529K  & --            & / & Sat.+Ground  & --        & --         & --         & --         & -- \\
GeoContext-v1   & 26K   & --            & / & Sat.+Ground  & --        & --         & --         & --         & -- \\
\bottomrule
\end{tabular}
\end{table}
